Generative Moment Matching Networks

We consider the problem of learning deep generative models from data. We formulate a method that generates an independent sample via a single feedforward pass through a multilayer perceptron, as in the recently proposed generative adversarial networks (Goodfellow et al., 2014). Training a generative adversarial network, however, requires careful optimization of a difficult minimax program. Instead, we utilize a technique from statistical hypothesis testing known as maximum mean discrepancy (MMD), which leads to a simple objective that can be interpreted as matching all orders of statistics between a dataset and samples from the model, and can be trained by backpropagation. We further boost the performance of this approach by combining our generative network with an auto-encoder network, using MMD to learn to generate codes that can then be decoded to produce samples. We show that the combination of these techniques yields excellent generative models compared to baseline approaches as measured on MNIST and the Toronto Face Database.

==> conclusion.tex <==
In this paper we provide a simple and effective framework for training deep
generative models called generative moment matching networks. Our approach is
based off of optimizing maximum mean discrepancy so that samples generated
from the model are indistinguishable from data examples in terms of their
moment statistics. As is standard with MMD, the use of the kernel trick allows
a GMMN to avoid explicitly computing these moments, resulting in a simple
training objective, and the use of minibatch stochastic gradient descent
allows the training to scale to large datasets.

Our second contribution combines MMD with auto-encoders for learning a
generative model of codes in the code layer.
%in order to generate samples of the encoding layer.
The code samples from the model can then be fed through the
decoder in order to generate samples in the original space. 
%Unlike previous
%methods, the use of auto-encoders in this situation provides an elegant way to learn
%complex distributions with a relatively simple learning algorithm. 
The use of auto-encoders makes the generative model learning a much simpler
problem. Combined with MMD, pretrained auto-encoders can be readily bootstrapped
into a good generative model of data.
On the
MNIST and Toronto Face Dataset, the GMMN+AE model achieves superior
performance compared to other approaches. For these datasets, we demonstrate
that the GMMN+AE is able to discover the implicit manifold of the data.

